FinLoRA: Benchmarking LoRA Methods for Fine-Tuning LLMs on Financial Datasets

Low-rank adaptation (LoRA) methods show great potential for scaling pre-trained general-purpose Large Language Models (LLMs) to hundreds or thousands of use scenarios. However, their efficacy in high-stakes domains like finance is rarely explored, e.g., passing CFA exams and analyzing SEC filings. In this paper, we present the open-source FinLoRA project that benchmarks LoRA methods on both general and highly professional financial tasks. First, we curated 19 datasets covering diverse financial applications; in particular, we created four novel XBRL analysis datasets based on 150 SEC filings. Second, we evaluated five LoRA methods and five base LLMs. Finally, we provide extensive experimental results in terms of accuracy, F1, and BERTScore and report computational cost in terms of time and GPU memory during fine-tuning and inference stages. We find that LoRA methods achieved substantial performance gains of 36\% on average over base models. Our FinLoRA project provides an affordable and scalable approach to democratize financial intelligence to the general public. Datasets, LoRA adapters, code, and documentation are available at https://github.com/Open-Finance-Lab/FinLoRA

==> tables/main_results_extended.tex <==

\newcommand{\af}[4]{%
  \makecell{% Args: #1 accuracy, #2 error, #3 f1, #4, confidence interval (ci)
    \textcolor{blue}{#1}\\% Accuracy
    \textcolor{blue}{\scriptsize CI: #2} \\ % Accuracy error
    \textcolor{blue}{\scriptsize std: #4} \\% Accuracy confidence interval
    \textcolor{gray}{#3} % F1
  }%
}

\newcommand{\bert}[4]{%
  \makecell{% Args: #1 no usage, leave 0.00 or empty. #2 bert f1 error, #3 bert f1, #4 bert f1 ci
    \textcolor{green}{#3} \\ % BERT F1
    \textcolor{green}{\scriptsize CI:#2} \\ % BERT f1 error
    \textcolor{green}{\scriptsize std: #4} % BERT f1 ci
  }%
}
\addtolength{\tabcolsep}{-0.4em} % Reduced tabcolsep further for more columns




% --- Parsed Data (for reference, not part of LaTeX output) ---
% This is a representation of the logic used to map your CSV data.
% parsed_data["FPB"]["Llama3.1 8B"] = ("1.434", "0.577")
% parsed_data["FPB"]["DeepSeekV3"] = ("1.434", "0.577")
% parsed_data["FPB"]["GPT4o"] = ("0.000", "0.000")
% ... and so on for all datasets and relevant models.
% For XBRL-Term, Gemini: parsed_data["XBRL-Term"]["Gemini2FL"] = ("0.559", "0.563")
% --- End of Parsed Data ---

\begin{table}[H] \small
\centering
\caption{Performance on General Financial Tasks: \textcolor{blue}{accuracy} in blue, \textcolor{gray}{F1} in gray, and \textcolor{green}{BERTScore F1} in green.}
% Adjusted tabular definition for 2 new base models: l|ccccccc|cccc|c
\begin{tabular}{l|ccccccc|cccc|c}
\toprule
% Adjusted multicolumn for 7 base models
\multirow{5}{*}{\bf Datasets} & \multicolumn{7}{c|}{\bf Base Models} & \multicolumn{5}{c}{\bf Fine-tuned Models} \\
% Adjusted cmidrule for 12 model columns (2 to 13)
\cmidrule(lr){2-13}
& Llama  & Llama & \makecell{FinGPT} & \makecell{Bloomberg\\GPT} & DeepSeek & GPT- & Gemini & Llama & Llama & Llama & Llama & Gemini \\
& 3.1 8B \cite{llama} & 3.1 70B  \cite{llama} & \cite{liu2023fingpt, wang2023fingptinstructiontuningbenchmark} & \cite{wu2023bloomberggpt} & V3 \cite{liu2024deepseek} & 4o \cite{hurst2024gpt} & 2.0 FL \cite{geminiteam2024geminifamilyhighlycapable} & 3.1 8B  & 3.1 8B  & 3.1 8B  & 3.1 8B  & 2.0 FL \\ 
&    &  &   &   &   &   &   & LoRA & QLoRA & DoRA & rsLoRA & N/A \\ 
&    &  &   &   &   &   &   & 8bit-r8 & 4bit-r4 & 8bit-r8 & 8bit-r8 & N/A \\ 
\midrule
\rowcolor{surface}
% Adjusted multicolumn for 13 total columns
\multicolumn{13}{c}{\bf General Financial Tasks} \\
\midrule
FPB 
& \af{68.73}{1.434}{0.677}{0.577} 
& \af{74.50}{-}{0.736}{-} 
& \af{-}{-}{0.861}{-} % FinGPT
& \af{51.07}{-}{-}{-} % BloombergGPT
& \af{78.76}{1.434}{0.764}{0.577} 
& \af{81.13}{0.000}{0.818}{0.000} 
& \af{81.02}{1.434}{0.894}{0.577} 
& \af{85.64}{0.000}{\textbf{0.922}}{0.000} 
& \af{84.16}{1.434}{0.909}{0.577} 
& \af{81.93}{0.000}{0.901}{0.000} 
& \af{82.84}{1.434}{0.853}{0.577} 
& \af{\textbf{87.62}}{0.000}{0.878}{0.000} \\ \addlinespace

\makecell[l]{FiQA SA} 
& \af{46.55}{1.434}{0.557}{0.577} 
& \af{47.27}{-}{0.565}{-} 
& \af{-}{-}{0.825}{-} 
& \af{75.07}{-}{-}{-} 
& \af{60.43}{2.484}{0.686}{1.000} 
& \af{72.34}{5.171}{0.773}{2.082} 
& \af{68.09}{0.000}{0.810}{0.000} 
& \af{81.28}{0.000}{\textbf{0.884}}{0.000} 
& \af{78.30}{0.000}{0.874}{0.000} 
& \af{78.72}{1.434}{0.874}{0.577} 
& \af{73.19}{0.000}{0.806}{0.000} 
& \af{\textbf{88.09}}{0.000}{0.879}{0.000} \\ \addlinespace

TFNS 
& \af{69.97}{1.434}{0.683}{0.577} 
& \af{68.42}{-}{0.686}{-} 
& \af{-}{-}{0.890}{-} 
& \af{-}{-}{-}{-} 
& \af{84.38}{0.000}{0.846}{0.000} 
& \af{73.32}{4.968}{0.740}{2.000} 
& \af{26.38}{0.000}{0.385}{0.000} 
& \af{88.02}{0.000}{\textbf{0.932}}{0.000} 
& \af{83.84}{1.434}{0.910}{0.577} 
& \af{59.09}{0.000}{0.702}{0.000} 
& \af{59.51}{2.868}{0.655}{1.155} 
& \af{\textbf{89.49}}{0.000}{0.896}{0.000} \\ \addlinespace

NWGI 
& \af{43.86}{2.484}{0.583}{1.000} 
& \af{50.14}{-}{0.596}{-} 
& \af{-}{-}{0.652}{-} 
& \af{-}{-}{-}{-} 
& \af{7.44}{0.000}{0.097}{0.000} 
& \af{66.61}{4.968}{0.656}{2.000} 
& \af{48.16}{1.434}{0.614}{0.577} 
& \af{54.16}{2.484}{\textbf{0.690}}{1.000} 
& \af{49.96}{0.000}{0.645}{0.000} 
& \af{19.57}{0.000}{0.281}{0.000} 
& \af{35.80}{1.434}{0.464}{0.577} 
& \af{\textbf{62.59}}{0.000}{0.581}{0.000} \\ \addlinespace

NER 
& \af{48.89}{0.000}{0.569}{0.000} 
& \af{46.28}{-}{0.454}{-} 
& \af{-}{-}{-}{-} 
& \af{60.82}{-}{-}{-} 
& \af{40.82}{0.000}{0.360}{0.000} 
& \af{52.11}{4.303}{0.523}{1.732} 
& \af{65.13}{0.000}{0.769}{0.000} 
& \af{\textbf{98.05}}{0.000}{\textbf{0.981}}{0.000} 
& \af{96.63}{0.000}{0.966}{0.000} 
& \af{71.59}{1.434}{0.834}{0.577} 
& \af{95.92}{0.000}{0.963}{0.000} 
& \af{97.29}{0.000}{0.973}{0.000} \\ \addlinespace

Headline 
& \af{45.34}{3.795}{0.558}{1.528} 
& \af{71.68}{-}{0.729}{-} 
& \af{-}{-}{-}{-} 
& \af{82.20}{-}{-}{-} 
& \af{76.06}{3.795}{0.779}{1.528} 
& \af{80.53}{1.434}{0.814}{0.577} 
& \af{76.60}{1.434}{0.847}{0.577} 
& \af{84.66}{0.000}{0.852}{0.000} 
& \af{88.03}{0.000}{0.886}{0.000} 
& \af{64.93}{1.434}{0.781}{0.577} 
& \af{71.75}{1.434}{0.828}{0.577} 
& \af{\textbf{97.32}}{0.000}{\textbf{0.973}}{0.000} \\ \addlinespace
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H] \small
\centering
\caption{Performance on Financial Certificate Tasks: \textcolor{blue}{accuracy} in blue, \textcolor{gray}{F1} in gray, and \textcolor{green}{BERTScore F1} in green.}
\begin{tabular}{l|ccccc|cccc|c} % No new models here, so structure is l|ccccc|cccc|c
\toprule
\multirow{5}{*}{\bf Datasets} & \multicolumn{5}{c|}{\bf Base Models} & \multicolumn{5}{c}{\bf Fine-tuned Models} \\
\cmidrule(lr){2-11} % Spans columns 2 through 11
& Llama & Llama & DeepSeek & GPT- & Gemini & Llama & Llama & Llama & Llama & Gemini \\
& 3.1 8B \cite{llama} & 3.1 70B  \cite{llama} & V3 \cite{liu2024deepseek} & 4o \cite{hurst2024gpt} & 2.0 FL \cite{geminiteam2024geminifamilyhighlycapable} & 3.1 8B  & 3.1 8B  & 3.1 8B  & 3.1 8B  & 2.0 FL \\ 
&    &  &   &   &   & LoRA & QLoRA & DoRA & rsLoRA & N/A \\ 
&    &  &   &   &   & 8bit-r8 & 4bit-r4 & 8bit-r8 & 8bit-r8 & N/A \\ 
\midrule
\rowcolor{surface}
\multicolumn{11}{c}{\bf Financial Certificate Tasks} \\
\midrule
\makecell[l]{CFA\\Level 1} 
& \af{13.33}{4.667}{0.133}{1.879} 
& \af{42.22}{-}{0.418}{-} 
& \af{54.44}{4.216}{0.556}{1.697} 
& \af{63.33}{1.595}{0.631}{0.642} 
& \af{55.56}{1.593}{0.556}{0.641} 
& \af{86.67}{1.593}{0.867}{0.641} 
& \af{\textbf{87.78}}{0.000}{\textbf{0.878}}{0.000} 
& \af{\textbf{87.78}}{1.593}{\textbf{0.878}}{0.641} 
& \af{\textbf{87.78}}{1.593}{\textbf{0.878}}{0.641} 
& \af{52.22}{2.757}{0.530}{1.110} \\ \addlinespace

\makecell[l]{CFA\\Level 2} 
& \af{19.48}{4.153}{0.199}{1.672} 
& \af{29.87}{-}{0.303}{-} 
& \af{46.75}{6.716}{0.485}{2.704} 
& \af{55.84}{1.863}{0.563}{0.750} 
& \af{56.67}{1.863}{0.567}{0.750} 
& \af{88.31}{3.725}{0.883}{1.499} 
& \af{83.12}{3.227}{0.835}{1.299} 
& \af{90.91}{6.453}{0.909}{2.598} 
& \af{\textbf{92.21}}{7.475}{\textbf{0.922}}{3.009} 
& \af{51.11}{1.864}{0.519}{0.751} \\ \addlinespace

\makecell[l]{CFA\\Level 3} 
& \af{16.67}{1.839}{0.179}{0.740} 
& \af{24.36}{-}{0.271}{-} 
& \af{47.44}{6.024}{0.496}{2.425} 
& \af{51.28}{3.677}{0.517}{1.480} 
& \af{52.56}{1.839}{0.538}{0.740} 
& \af{70.51}{5.516}{0.705}{2.220} 
& \af{66.67}{6.629}{0.675}{2.669} 
& \af{69.23}{3.185}{0.697}{1.282} 
& \af{\textbf{79.49}}{1.839}{\textbf{0.795}}{0.740} 
& \af{51.28}{1.850}{0.557}{0.745} \\ \addlinespace

\makecell[l]{CPA\\REG} 
& \af{31.68}{2.459}{0.317}{0.990} 
& \af{41.58}{-}{0.426}{-} 
& \af{65.35}{1.420}{0.654}{0.572} 
& \af{67.33}{2.841}{0.667}{1.144} 
& \af{63.37}{1.420}{0.638}{0.572} 
& \af{80.20}{1.420}{0.802}{0.572} 
& \af{88.12}{2.840}{0.885}{1.143} 
& \af{\textbf{90.10}}{0.000}{\textbf{0.901}}{0.000} 
& \af{\textbf{90.10}}{0.000}{\textbf{0.901}}{0.000} 
& \af{51.28}{1.420}{0.557}{0.572} \\ \addlinespace 
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H] \small
\centering
\caption{Performance on Financial Reporting Tasks: \textcolor{blue}{accuracy} in blue, \textcolor{gray}{F1} in gray, and \textcolor{green}{BERTScore F1} in green.}
% Adjusted tabular definition for 1 new base model: l|cccccc|cccc|c
\begin{tabular}{l|cccccc|cccc|c}
\toprule
% Adjusted multicolumn for 6 base models
\multirow{5}{*}{\bf Datasets} & \multicolumn{6}{c|}{\bf Base Models} & \multicolumn{5}{c}{\bf Fine-tuned Models} \\
% Adjusted cmidrule for 11 model columns (2 to 12)
\cmidrule(lr){2-12}
& Llama & Llama & \makecell{SEC-\\BERT} & DeepSeek & GPT- & Gemini & Llama & Llama & Llama & Llama & Gemini \\
& 3.1 8B \cite{llama} & 3.1 70B  \cite{llama} & \cite{loukas-etal-2022-finer, fnxl} & V3 \cite{liu2024deepseek} & 4o \cite{hurst2024gpt} & 2.0 FL \cite{geminiteam2024geminifamilyhighlycapable} & 3.1 8B  & 3.1 8B  & 3.1 8B  & 3.1 8B  & 2.0 FL \\ 
&    &  &   &   &   &   & LoRA & QLoRA & DoRA & rsLoRA & N/A \\ 
&    &  &   &   &   &   & 8bit-r8 & 4bit-r4 & 8bit-r8 & 8bit-r8 & N/A \\ 
\midrule
\rowcolor{surface}
% Adjusted multicolumn for 12 total columns
\multicolumn{12}{c}{\bf Financial Reporting Tasks} \\
\midrule
FiNER 
& \af{21.28}{3.420}{0.232}{1.377} 
& \af{61.82}{-}{0.606}{-} 
& \af{-}{-}{-}{-} % SEC-BERT
& \af{68.92}{3.187}{0.699}{1.283} 
& \af{72.29}{2.351}{0.725}{0.946} 
& \af{63.91}{0.359}{0.638}{0.144} 
& \af{74.10}{2.151}{0.759}{0.866} 
& \af{74.32}{0.949}{0.760}{0.382} 
& \af{70.92}{5.171}{0.732}{2.082} 
& \af{70.72}{5.171}{0.724}{2.082} 
& \af{\textbf{80.32}}{0.000}{\textbf{0.802}}{0.000} \\ \addlinespace

FNXL 
& \af{3.64}{2.868}{0.045}{1.155} 
& \af{20.14}{-}{0.210}{-} 
& \af{-}{-}{46.20}{-} 
& \af{27.33}{2.800}{0.288}{1.127} 
& \af{42.41}{2.351}{0.398}{0.946} 
& \af{37.75}{2.151}{0.356}{0.866} 
& \af{23.57}{1.897}{0.250}{0.764} 
& \af{23.05}{0.717}{0.253}{0.289} 
& \af{33.50}{1.434}{0.311}{0.577} 
& \af{35.68}{1.242}{0.348}{0.500} 
& \af{\textbf{47.98}}{0.000}{\textbf{0.438}}{0.000} \\ \addlinespace

\makecell[l]{XBRL\\Term} 
& \bert{-}{ 0.002}{0.574}{0.001} 
& \bert{-}{ -}{0.587}{-} 
& \bert{-}{ -}{-}{-} 
& \bert{-}{ 0.001}{0.573}{0.001} 
& \bert{-}{ 0.002}{0.584}{0.001} 
& \bert{-}{0.559}{0.572}{0.563} 
& \bert{-}{ 0.004}{0.599}{0.002} 
& \bert{-}{ 0.003}{0.606}{0.001} 
& \bert{-}{ 0.017}{0.606}{0.007} 
& \bert{-}{ 0.002}{0.630}{0.001} 
& \bert{-}{ 0.000}{\textbf{0.666}}{0.000} \\ \addlinespace
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H] \small
\centering
\caption{Performance on Financial Statement Analysis Tasks: \textcolor{blue}{accuracy} in blue, \textcolor{gray}{F1} in gray, and \textcolor{green}{BERTScore F1} in green.}
\begin{tabular}{l|ccccc|cccc|c} % No new models here
\toprule
\multirow{5}{*}{\bf Datasets} & \multicolumn{5}{c|}{\bf Base Models} & \multicolumn{5}{c}{\bf Fine-tuned Models} \\
\cmidrule(lr){2-11}
& Llama  & Llama & DeepSeek & GPT- & Gemini & Llama & Llama & Llama & Llama & Gemini \\
& 3.1 8B \cite{llama} & 3.1 70B  \cite{llama} & V3 \cite{liu2024deepseek} & 4o \cite{hurst2024gpt} & 2.0 FL \cite{geminiteam2024geminifamilyhighlycapable} & 3.1 8B  & 3.1 8B  & 3.1 8B  & 3.1 8B  & 2.0 FL \\ 
&    &  &   &   &   & LoRA & QLoRA & DoRA & rsLoRA & N/A \\ 
&    &  &   &   &   & 8bit-r8 & 4bit-r4 & 8bit-r8 & 8bit-r8 & N/A \\ 
\midrule
\rowcolor{surface}
\multicolumn{11}{c}{\bf Financial Statement Analysis Tasks} \\
\midrule
\makecell[l]{Tag \\ Extraction} 
& \af{69.16}{3.795}{0.739}{1.528} 
& \af{69.64}{-}{0.782}{-} 
& \af{85.03}{2.484}{0.849}{1.000} 
& \af{81.60}{7.589}{0.864}{3.055} 
& \af{80.27}{0.000}{0.811}{0.000} 
& \af{\textbf{89.13}}{6.572}{0.886}{2.646} 
& \af{86.89}{5.171}{0.872}{2.082} 
& \af{80.44}{8.957}{0.896}{3.606} 
& \af{85.26}{2.868}{0.879}{1.155} 
& \af{85.03}{0.000}{\textbf{0.907}}{0.000} \\ \addlinespace

\makecell[l]{Value \\ Extraction} 
& \af{52.46}{3.795}{0.565}{1.528} 
& \af{88.19}{-}{0.904}{-} 
& \af{98.01}{0.000}{0.982}{0.000} 
& \af{97.01}{0.000}{0.974}{0.000} 
& \af{98.02}{0.000}{0.980}{0.000} 
& \af{98.49}{0.000}{0.986}{0.000} 
& \af{97.14}{0.000}{0.974}{0.000} 
& \af{98.57}{0.000}{0.988}{0.000} 
& \af{99.13}{0.000}{\textbf{0.992}}{0.000} 
& \af{\textbf{99.20}}{0.000}{\textbf{0.992}}{0.000} \\ \addlinespace

\makecell[l]{Formula \\ Construction} 
& \af{12.92}{4.303}{0.201}{1.732} 
& \af{59.28}{-}{0.665}{-} 
& \af{22.75}{4.303}{0.315}{1.732} 
& \af{79.76}{1.434}{0.820}{0.577} 
& \af{61.90}{0.000}{0.644}{0.000} 
& \af{77.61}{5.737}{0.876}{2.309} 
& \af{89.34}{4.303}{\textbf{0.898}}{1.732} 
& \af{88.02}{6.572}{0.882}{2.646} 
& \af{\textbf{89.46}}{5.737}{0.893}{2.309} 
& \af{67.85}{0.000}{0.786}{0.000} \\ \addlinespace

\makecell[l]{Formula\\Calculation} 
& \af{27.27}{3.795}{0.317}{1.528} 
& \af{77.49}{-}{0.783}{-} 
& \af{85.99}{0.000}{0.868}{0.000} 
& \af{83.59}{1.434}{0.857}{0.577} 
& \af{53.57}{0.000}{0.536}{0.000} 
& \af{98.68}{0.000}{0.990}{0.000} 
& \af{92.81}{1.434}{0.947}{0.577} 
& \af{\textbf{98.92}}{0.000}{\textbf{0.993}}{0.000} 
& \af{98.80}{0.000}{0.988}{0.000} 
& \af{54.76}{0.000}{0.548}{0.000} \\ \addlinespace

\makecell[l]{Finance\\Bench} 
& \bert{-}{ 0.008}{0.443}{0.003} 
& \bert{-}{ -}{ 0.528}{-} 
& \bert{-}{ 0.007}{0.573}{0.003} 
& \bert{-}{ 0.017}{0.564}{0.007} 
& \bert{-}{ 0.007}{0.552}{0.003} 
& \bert{-}{ 0.007}{0.511}{0.003} 
& \bert{-}{ 0.017}{0.542}{0.007} 
& \bert{-}{ 0.014}{0.477}{0.006} 
& \bert{-}{ 0.014}{\textbf{0.575}}{0.006} 
& \bert{-}{ 0.000}{0.544}{0.000} \\ \addlinespace

\makecell[l]{Financial\\Math} 
& \af{11.00}{3.795}{0.136}{1.528} 
& \af{10.50}{-}{0.134}{-} 
& \af{21.50}{1.434}{0.255}{0.577} 
& \af{27.00}{1.434}{0.296}{0.577} 
& \af{19.00}{1.434}{0.204}{0.577} 
& \af{30.00}{1.434}{0.332}{0.577} 
& \af{26.50}{1.434}{0.307}{0.577} 
& \af{28.50}{2.868}{0.317}{1.155} 
& \af{34.50}{1.434}{0.370}{0.577} 
& \af{\textbf{66.00}}{0.000}{\textbf{0.785}}{0.000} \\ \addlinespace
\bottomrule
\end{tabular}
\end{table}


